Programming Scalable Cloud Services with AEON

Designing low-latency cloud-based applications that are adaptable to unpredictable workloads and efficiently utilize modern cloud computing platforms is hard. The actor model is a popular paradigm that can be used to develop distributed applications: actors encapsulate state and communicate with each other by sending events. Consistency is guaranteed if each event only accesses a single actor, thus eliminating potential data races and deadlocks. However it is nontrivial to provide consistency for concurrent events spanning across multiple actors. This paper addresses this problem by introducing AEON: a framework that provides the following properties: (i) Programmability: programmers only need to reason about sequential semantics when reasoning about concurrency resulting from multi-actor events; (ii) Scalability: AEON runtime protocol guarantees serializable and starvation-free execution of multi-actor events, while maximizing parallel execution; (iii) Elasticity: AEON supports fine-grained elasticity enabling the programmer to transparently migrate individual actors without violating the consistency or entailing significant performance overheads. Our empirical results show that it is possible to combine the best of all the above three worlds without compromising on the application performance.

==> Overview.tex <==
\section{Motivating Example and Overview}
\label{sec:overview}
%
% Any correct and scalable distributed cloud application must explcitly implement the logic for concurrent processing of application operations
% and handle migration of both data and computation between
% nodes in case of a change in the workload.
% However, writing even
% simple applications which meet the desired scalability criteria would
% require expert programmers in distributed systems. Even in that case,
% it would remain an error prone, time consuming and expensive endeavor.


Let us introduce the main components of  \aeon{} through a
simple example.  We consider an application \'{a}-la \emph{\Piazza{}}~\cite{Piazza}, an online service that allows instructors
and students to organize a class by allowing students to register in
classes, interact with each other and the instructor through a
forum-like environment, etc.

%\begin{figure}[!t]
\begin{lstlisting}[caption=\aeon{} code snippet,float,label=aeon-implementation,basicstyle=\footnotesize\ttfamily,captionpos=b,frame=b,escapechar=|]
context Course events <snow_day, ...> {|\label{line:Course}|
  vector<Person> students;         // students|\label{line:students}|
  vector<Person> instructors;    // instructor
  ... 
  void snow_day() {
    // update student tokens in parallel
    for(int i=0 upto students.size())
      async students[i]->add_tokens(1);|\label{line:add_tokens}|
    // notify all instructors atomically
    for( int i=0 upto instructors.size())
      instructors[i]->notify("Snow-Day");|\label{line:notify}|
    ...
  }
}
context Person events <use_token, ...> {|\label{line:Person}|
  Role role; // staff or student|\label{line:role}|
  int tokens; // tokens
  ... 
  void add_tokens(int n) {
    tokens =+ n;
  } 
  void use_token() {
    tokens =- 1;
  }
  bool notify(String str) { ... }

}
class Role { ... }|\label{line:Role}|
context University ... {|\label{line:University}|
  vector<Department> departments; ...
}
context Department ... {|\label{line:Department}|
  vector<Course> Courses; ...
}
...
\end{lstlisting}
%\vspace{-\topsep}  
%\end{figure}

\vspace{1mm}\noindent\textbf{Scenario.}~ Consider that we are interested in providing the following
functionality. We have a course where students have multiple
assignments that they have to turn in on predefined deadlines. The
students are allowed a total of $n$ days of delays throughout the
semester. To that end, they are initially given $n$ tokens, each of
which they can trade for one day of delay. Moreover, to cover for
eventualities such as a cancelled lab or class, an additional token
can be given to each student concerned.
The addition of tokens can only be triggered by a teaching assistant
(TA), or an instructor of the class. Moreover, we must guarantee that
each of the TAs and instructors are immediately notified of the
addition of tokens (otherwise they might repeat the operation).

Since students can decide asynchronously at any point to use a token,
the programmer must guarantee that upon a token-increment event, the
tokens of each student are updated atomically (to avoid the risk of a
student obtaining extra tokens through a race condition). Moreover,
the token increment event must be made visible immediately -- or
rather atomically -- to all TAs and instructors in the course.

\autoref{aeon-implementation} outlines a possible implementation of this scenario in \aeon{}, which is implemented as an extension of C++. 
We remark that keywords appearing in red color are new to \aeon{}, and we use the syntactic form
\lstinline{upto} to iterate through a numerical range.  We will
elaborate on the example by providing intuitions about the different
constructs, which will be further explained in~\autoref{sec:pmodel}.

\vspace{1mm}\noindent\textbf{Contexts.}~ 
The declarations of contexts at lines~\autoref{line:Course}
and~\autoref{line:Person} can be thought of as class-like foundries for distributed objects with the
following characteristics: 
\begin{inparaenum}[(i)]
\item They can contain data in the form of fields. As customary such fields can
  be of class types, as is the case of line~\ref{line:role}
  declaring a field \lstinline|role|, an instance of the class \lstinline|Role|
  declared at line~\ref{line:Role}. In this case, the class instance
  \lstinline|role| is guaranteed to reside in the same server as the
  context instance of \lstinline|Person| that refers to
  it. 
\item Alternatively, they can contain references to \emph{context
    instances}.  For instance at line~\ref{line:students}, the field
  \lstinline|students| contains a vector holding references to
  \lstinline|Person| context instances, which possibly reside on different
  hosts. %Notice that much like classes in \Java{} or
 % \cpp{}, context declarations define types.
\end{inparaenum}

While contexts are roughly analogous to distributed classes in frameworks
like~\rmi{}~\cite{RMI99} or \corba{}~\cite{CORBA3}, 
\aeon{} context instances are automatically migrated by the \aeon{}
runtime system. %, relieving the programmer from such decisions. 
More differences affecting the use of context instances to facilitate such migration 
will be explained shortly in \autoref{sec:pmodel}.

% \gp{Not sure if this is the place to talk about the DAG structure of
%   contexts.}

% In this section,we elaborate on these problems and our solution, \emph{i.e.}, \aeon with an example
% application, namely, \emph{\Piazza{}}, an online application that
% allows instructors and students to organize a class~\cite{Piazza}. 
% Instructors can disseminate materials, make announcements, and answer
% students questions. 
% Students registered in an actual class of a university can register in
% the \Piazza{} forum created for the class, and they can ask and respond
% questions in a forum like environment where the turnaround for answers
% might be much faster than if they had to wait for a face-to-face
% interaction.

\vspace{1mm}\noindent\textbf{Events and calls.}~ Like other
environments to write Internet-facing
applications (e.g.,~\cite{BykovGKLPT11,ChuangSYGKK13}), \aeon{} follows an event-driven model, 
where clients of the system interact with the
server application by issuing events to the latter (cf. \autoref{fig:application}). Contexts
(lines~\ref{line:Course} and~\ref{line:Person}) declare which of
their methods can be directly called by clients as events. Importantly, the execution of an individual event is guaranteed to be atomic -- more precisely, linearizable with respect to other events. The
declaration of which methods can be used as an event is achieved
through the \lstinline|events| keyword in the declaration of
contexts.
%\footnote{We could alternatively provide a specific interface
%  to declare events as in the case of \rmi{}. We use
%  \lstinline|events| for succinctness.}
%

Notice for instance at line~\ref{line:Person} that while
\lstinline|use_token| is declared as an event, \lstinline|add_tokens|
is not, since the latter can only be called as part of an event
executing in the course context (initiated by a TA or an instructor). 
As it has been foreshadowed, context methods can call other context
methods. The argument passing convention is that context instances
are passed by reference, while objects are passed by value, i.e., deep copying.  
%Notice that passing classes by-value posses no problem
%since class instances cannot contain context references.

In particular, other than event calls, which are generally reserved
for ``external'' calls from clients to the main application, context method calls can be either
synchronous -- the implicit assumption -- or asynchronous, indicated
with the \lstinline|async| keyword at the call site. Evidently, a
synchronous call blocks the execution of the event in the current
context until a result is obtained from the target context upon
return. 
Line~\ref{line:notify} shows an example of a synchronous context call, which needs to wait for a boolean response
indicating if the notification was successfully processed or
not (code elided for brevity). 
%
Conversely asynchronous calls do not wait for a result, and
allow execution to proceed immediately, hence allowing for parallel
execution of methods called.  An example of asynchronous call is
given at line~\ref{line:add_tokens}. In this case, the execution of
the \lstinline|add_tokens| method in one student needs not wait for
all prior calls to \lstinline|add_tokens| in other students. We
require that asynchronous calls be only made on methods without return values
%procedures (as opposed to functions)
, but this %unimportant 
restriction could be easily lifted
by introducing \emph{futures}~\cite{YBS86}, which we do not do at the moment.



% \input{old-overview}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> PM.tex <==
\section{The \aeon{} Model}
\label{sec:programming-model}

\gustavo{List of things that I would say here:}

\aeon{} is an attempt to strike a compromise between the challenges
outlined in the previous sections: programmability, scalability and
elasticity.

\aeon{} program design is centered around the following notions:
\begin{itemize}
\item (Programability) The underlying programming paradigm of \aeon{}
  is \emph{Object-Orientated} (OO). We believe that a familiar OO
  programming model, which most programmers learn in their first courses
  in any programming curriculum, guarantees that the learning curve of
  \aeon{} is steep (easy to learn). Moreover, a programmer new to
  \aeon{} should only be concerned with the specific aspects related to
  distribution and elasticity.
\item (Scalability, Elasticity) \emph{Contexts}. The notion of context
  is a natural extension of the notion of objects in OO. However,
  contexts, and their instances \emph{places??} carry a connotation of
  distribution and mobility. In a nutshell, places represent instances
  of data structures that can be distributed among the computational
  resources of the runtime environment. Moreover, places can be migrated
  to accomodate for different workloads, hence achieving elasticity.
  \begin{itemize}
  \item Contexts, like objects, encapsulate both data and
    functionality. Unlike objects however, the representation of an object
    (it's fields) is inaccessible outside the scope of the contest. This
    is similar to the \smalltalk{} enforcement of representation
    hiding. Therefore, the only way to interact with places is through the
    methods (messages in OO parlance) provided by their interface.
  \item A whole place is the minimal unit of migration and
    distribution in \aeon{}. This means that the representation of a place
    resides in a single (albeit, not always the same) computational
    resource at all times. It is therefore important to design contexts
    with an appropriate granularity guaranteeing at the same time that the
    computational resources are not exhausted, and at the same time that
    no unnecessary overhead is added by an overpopulation of contexts.
  \item Also unlike objects, places are distributed and migratory,
    meaning that their communication patterns have to be restricted to
    guarantee a viable performance under the assumption that potentially
    each call into a place might represent a roundtrip in the
    network. Therefore, we adopt a multi-ownership structure that
    restricts method calls from a place to another if the latter is a
    child context of the former.
  \end{itemize}
\end{itemize}

%%% TeX-master: "main"
%%% Local Variables: 
%%% mode: latex 
%%% TeX-master: "main" 
%%% End:


==> Scalability.tex <==
\section{Implementation}
\label{sec:scalability}
We implemented \aeon on top of Mace~\cite{mace}, a C\texttt{++} language
extension that provides a unified framework for network communication and event handling.
%Based on Mace~\cite{mace} framework, we build up this new model with around
The implementation of \aeon{} consists in roughly 10,000 lines of core code and 110 new classes on top of Mace. 
%
Due to space constraints we focus on briefly discussing (i) how scalability is increased through parallelism and scale adjustment 
and (ii) fault tolerance.
%in two ways: (i) \aeon
%employs several techniques to maximize the parallelism in the execution of
%different events, thus exploiting the distributed nature of cloud computing
%infrastructure; (ii) the runtime system attempts to optimize data center
%resources to maximize automatic scale adjustment while remaining economic.  solution.

\vspace{1mm}\noindent\textbf{Parallelism.}
%\aeon{} exploits several sources to increase parallelism. Firstly, 
The
ownership network of context instances already implies that %we can, at runtime, know
%when two context instances have common descendants. Then, 
whenever two events
target context instances that do not share descendants, they can execute in parallel and independently as shown
in~\autoref{sec:semantics} (cf. \autoref{th:indevents}).

Moreover, the runtime of \aeon{} puts in place an optimization over the
semantics presented in~\autoref{sec:semantics} for the case where two events target context instances that share only
a subset of descendant context instances. Here, the serialization achieved by locking the dominator
in~\autoref{sec:inter-cont-semantics} does not prevent the event arriving later (failing to acquire the dominator lock) from starting to execute on context instances that
are unshared. This optimization is clearly \emph{safe} since the latter event
will not attempt to acquire the context instances that are shared by the two targets,
therefore preventing the possibility of the former event being delayed by it,
and more importantly, avoiding the possibility of deadlock.\footnote{Notice
  that this is merely an optimization, and it does not affect the semantics
  of~\autoref{sec:semantics}.} This implies that if an event does not manage to
  acquire the lock
of the dominator, but does not attempt to access any context instances that are descendants shared 
with the target of the event currently holding the common dominator,
the event can complete.

%Finally, an additional mechanism that is put in place to maximize
%concurrency are the \emph{readonly} methods, which as it was shown
%in~\autoref{sec:inter-cont-semantics}, allows the execution of multiple
%concurrent readonly methods in a single event at the same time. 

\vspace{1mm}\noindent\textbf{Automatic scale adaption.}
\aeon{} runtime implements a \emph{scale manager} (\cservice{}) to manage
global information and operation.
\aeon{}'s \cservice{} delivers two capabilities:
\begin{inparaenum}[(i)]
    \item maintaining the global \emph{context map} (a data structure mapping context instances to servers) and ownership
    network, and \item automatic scale-adjustment by managing the context instances creation and migration.
\end{inparaenum}
Fault-tolerance of the \cservice{} is achieved through state machine
replication~\cite{Lamport1984}.

The \cservice{} follows the following protocol to migrate a context instance
 $\acontext$ from a host $s_1$ to a new host $s_2$:
% \begin{figure}[!h] %\frametitle{Migrate context $C$ from server $s_1$ to
% $s_2$}
\begin{inparaenum}[(1)] \item The \cservice{} sends a \emph{prepare} message to
  $s_2$, notifying that requests for context instance $\acontext$ might start arriving.
  Then, $s_2$ responds by creating a queue for context instance $\acontext$ and
  acks the \cservice{}.
  % \item[\textit{Step 2:}] $s_2$ creates an execution queue for enqueuing
  % events targeted to context $c$, and acknowledges the \cservice.
  \item
    Upon receiving the ack, the \cservice{} informs $s_1$ to stop
    receiving \event{s} targeting $\acontext$ and waits for $s_1$'s ack.
  % \item[\textit{Step 4:}] Upon receiving the stop request from the
  % \cservice{}, $s_1$ stops accepting new \events{} targeting context $c$ and
  % acknowledges it to the \cservice{}.
  \item Once the \cservice{} receives the ack, it updates its context mapping,
  assigning $C$ to $s_2$. % Thus, from this point on,
  % the \cservice{} returns $s_2$ as the location of context $c$.
  It then sends a special \event{} called
  \emph{$\textit{migrate}(\acontext,s_2)$} to $s_1$ indicating that $\acontext$
  has to be migrated to $s_2$.
  \item Upon receiving $\textit{migrate}(\acontext,s_2)$, $s_1$ enqueues an
  event $\textit{migrate}_{\acontext}$ in $\acontext.\aqueue$. This event serves
  as a notification for context instance $\acontext$ that it must migrate.
  When $\textit{migrate}_{\acontext}$ reaches the head of $\acontext.\aqueue$,
  $s_1$ spawns a thread to move $\acontext$ to $s_2$.
  \item
   Upon completion of the migration, $s_2$ notifies
  the \cservice{} that the migration is finished, and starts executing the
  enqueued events for context instance $\acontext$.
\end{inparaenum}
Observe that this simple protocol trivially ensures correctness during migrations
while still not stalling execution across all context instances.
As we show in \autoref{app:elas}, the performance penalty induced by
our migration protocol is limited.

\vspace{1mm}\noindent\textbf{Fault tolerance.} Fault tolerance of the \cservice{} is achieved through state machine
replication~\cite{Lamport1984} for high availability. %, which will automatically checkpoint its latest state.
\aeon{} provides programmers with a \lstinline|snapshot| API to handle faults in application components. In short, it allows 
programmers to take consistent snapshots of a given context instance and
all its children. To this end, and upon receiving a snapshot
request for a context instance, the \aeon{} runtime system dispatches a particular
event called \emph{snapshot event} to that context instance. 
%Consequently, this
%event takes consistent 
Snapshots of context instances and their children are achieved by writing them into a persistent
storage. To improve performance, a programmer is able
to override a method returning the state of a context. In case
the overridden method returns \lstinline!null! for a context instance, the runtime
system will ignore it during the checkpointing phase.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> algo-aeon.tex <==
\begin{algorithm*}[!t]
\caption{ \aeon{} event execution and synchronization}
\label{alg:aeon}

\begin{algorithmic}[1]
\begin{multicols}{2}
  	{\footnotesize

\Part{Event}{
    \State  $\ms{eid}$ \quad\Comment{unique event id}
    \State  $\ms{dom}$ \quad\Comment{dominator context}
    \State  $\ms{target}$ \quad\Comment{context the event lands}
    \State  $\ms{accessMode}$ \quad\Comment{indicate readonly or not}
}\EndPart

\Part{Context}{
    \State  $\ms{cid}$ \quad\Comment{unique id of the context}
    \State  $\ms{newEventqueue}$ \quad\Comment{queue for incoming events}
    \State  $\ms{queue}$ \quad\Comment{queue for executing events}
    \State  $\ms{lockQueue}$ \quad\Comment{map from contexts to events accessing the context}
}\EndPart

\Statex
\Part{acceptEvent(Event $E$)}{\quad\Comment{accept incoming event}
\State  $G  \gets \lit{getownershipnetwork()}$ \quad\Comment{return context graph}
\State  $\ms{dom} \gets G.\lit{getDom(E.target)}$ \quad\Comment{get dominator of context}
\State  $\ms{E.dom} \gets \ms{dom}$
\State  $\ms{dom}.\ms{newEventqueue}.\lit{enqueue(E)}$ \quad\Comment{add event in dominator incoming queue}
}\EndPart

\newpage

\Part{dispatchEvent(Context $C$)}{ \quad\Comment{dispatch next incoming event}
\State  {\bf wait}(!$C.\ms{newEventqueue}.\lit{isEmpty}()$)
\State  $G  \gets \lit{getownershipnetwork()}$
\State $E \gets C.\ms{newEventqueue}.\lit{dequeue}()$
\ForAll{($\ms{cid} \in G.\lit{reachableContexts}(\ms{E.target})$)} \quad\Comment{get descendants of context}
  \State  $\ms{lockQueue}[\ms{cid}].\lit{enqueue}(E.eid)$ 
\EndFor
\State $C' \gets E.\ms{target}$ 
\State  $C'.\ms{queue}.\lit{enqueue}(E)$ \quad\Comment{add in executing queue of target context} 
}\EndPart

\Statex

\Part{requestAccess(Event $E$, Context $C$)}{  \label{alg::aeon::lock}
\If {($E.\ms{accessMode}=$ READONLY)} \quad\Comment{readonly event only wait for exclusive events before it}
  \For {($\ms{E_0} \in \ms{lockQueue}[C.\ms{cid}].\lit{prefix}(E)$)} 
    \If {($\ms{E_0}.\ms{accessMode} =$ EXCLUSIVE)}
    \State {\bf wait}($E_0 \notin  \ms{lockQueue}[C.\ms{cid}]$)
    \EndIf
  \EndFor
  \Else\ {\bf wait}($\ms{lockQueue}[C.\ms{cid}].\lit{top}() = E.\ms{eid}$) \quad\Comment{reach head of queue to get access}
\EndIf}
\EndPart

\Statex

\Part{scheduleNext(Context $C$)}{ \quad\Comment{context C schedules next executing event}
\State {\bf wait}(!$C.\ms{queue}.\ms{isEmpty}()$)
\State  Event $E \gets C.\ms{queue}.\lit{dequeue}()$ 
\State  $E.\ms{dom}.\lit{requestAccess}(E, C)$ \label{line:access}
\State  $\lit{execute}(E)$ \quad\Comment{Execute event after access is granted}
}\EndPart
}\end{multicols}
\end{algorithmic}  
\end{algorithm*}


==> elas-extra.tex <==
\begin{figure*}[t]

  \centering
\subfloat[Average request latency]{\label{fig:memcached_latency}
  \includegraphics[width=.32\textwidth]{evaluation/memcached-latency.pdf}}
\subfloat[Server utilization]{\label{fig:memcached_servers}
  \includegraphics[width=.32\textwidth]{evaluation/memcached-servers.pdf}}
\subfloat[Pricing]{\label{fig:memcached_cost}
  \includegraphics[width=.32\textwidth]{evaluation/memcached-cost.pdf}}
\caption{Elasticity}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Scale Adjustment Experiments}\label{app:elas}
\Memcached{} is a popular key-value memory caching system
for web applications~\cite{memcached}.
%The implementation consists of multiple servers, all independent from each
%other.
%The client determines the server which holds a desired key-value pair via a hashing
%function of the \memcached{} library on the client's side and can then send a
%request to the server.
%If the server has the value in memory, it responds immediately;
%otherwise it retrieves the value from a permanent storage (e.g., a database) and
%then returns it to the client.
Generally, the cache miss rate is determined by both the capacity of the
\memcached{} servers and the workload.
For a fixed number of servers, the memory capacity is clearly bounded.
When the workload exceeds the memory capacity, the cache miss rate will increase
and more requests will be directed to permanent storage, downgrading the overall
performance.
So the ideal solution is to add and remove memory capacity according to the
workload, which could be done by an elastic \memcached{}.

% \vspace{-1em}
\vspace{1mm}\noindent\textbf{{\footnotesize\aeontitle{}} \Memcached{} and \Memcached{}.}~
%Since \memcached{} needs to
%have fixed identities for nodes, it does not adapt well to elastic applications,
%where contexts might migrate between different nodes.
We have implemented an elastic \memcached{} using \aeon{}. Unlike the standard
\memcached{}, our implementation is similar to a standard write-back cache
mechanism, where the last used key-value is stored into the persistent memory to
optimize the memory of the system. That is, clients do not know if there is a cache miss.

%a priori which
%host has the key-value copy, but the \aeon{} servers keep key-value pairs in
%memory following a least-used reclamation policy to evict key-values from the
%memory.

We set up our experiment on Amazon EC2 m1.medium instances with
128 clients over 16 instances. The size of a key-value pair is 1KB on
average. The client will repeatedly pick a random key and send a read
request to the \memcached{} system.
We vary the number of active clients over time.
The \aeon{} \memcached{} has 16 tables to store key-value pairs.
Therefore, \textit{table contexts} can be migrated into up to 16
servers according to the number of active clients.

For comparison we also implemented standard \memcached{}, in
which all servers are independent from each
other, and clients decide which server holds the pair.
The workload setup for the standard \memcached{} (the inelastic
version) is the same as elastic \memcached{}.

We run the experiment using \aeon{}, standard \memcached{} with 5 servers, and
standard \memcached{} with 17 servers (one server is used as permanent storage).
Figure \ref{fig:memcached_latency} plots the average latency for each of the
systems.
The number of active clients (muavae lines) is increased and
then decreased, in two rounds. During the first round, the latency of the three versions has a similar shape since all of
them require some warm-up time to retrieve the pairs from the persistent memory.
In the second round we can observe a more notorious performance gap.
For standard \memcached{} with 5 servers, 64 clients clearly exceed its capacity and a
high cache miss rate results in increased latency. Standard \memcached{} with 17
servers offers enough memory to handle the workload, so it can keep the average
latency at a very low level.
On the other hand, the capacity (i.e., the number of servers) varies based on
immediate workload for \aeon{} \memcached{}.
% \gpwarning{It is a bit unsatisfactory that AEON looks similar in both
%   rounds, whereas \memcached{} with 17 servers looks much better.}
Note that there are some short spikes for \aeon{} in
Figure~\ref{fig:memcached_latency}. These are caused by
the migration of contexts, as explained earlier.

Figure~\ref{fig:memcached_servers} shows the server utilization of
\aeon{} \memcached{}. It starts with 5 servers, increases first to
9 and then to 17, before decreasing inversely; then the whole
process repeats.
While the latency of \aeon{} \memcached{} is higher than that of \memcached{}
with 17 servers, the monetary cost of the latter is fixed for 17 servers for
the duration of the experiment and thus higher, although the 17 servers are only required for
two short periods of time. On the other hand, through elasticity, we
successfully obtained good performance with acceptable cost with
\aeon{}. This is shown in Figure~\autoref{fig:memcached_cost}, which shows the cost of
running \aeon{} \memcached{} and standard \memcached{} with 5 and 17 servers.
Since EC2 charges users hourly, and because we could not run our experiments
for hours, we reproduced that argument on a per second rate.
Figure~\autoref{fig:memcached_cost} shows that the cost of
\memcached{} with 17 servers is about \$0.35 for 50 seconds while \aeon{}
\memcached{} is charged only \$0.2 for the same duration.
%
Observe that when \aeon{} elastic Memcached scales out to 17 servers
(Figure~\autoref{fig:memcached_servers}), its latency is still higher than
17-server Memcached (Figure~\autoref{fig:memcached_latency}).
This is because the newly added servers need some time to populate
their cache lines.

\vspace{1mm}\noindent\textbf{Amazon ElastiCache.}~ We also compared \aeon{} \memcached{} to the
elastic version of \memcached{} implemented by \Amazon{}, called ElastiCache.
We have the following experiment setup:
\begin{inparaenum}
  \item \aeon{} \memcached{}: we run \aeon{} \memcached{} on 8
    Amazon EC2 m1.xLarge instances.
  \item ElastiCache: we create a \memcached{} cluster with 8
    Amazon E2 cache.m3.xLarge instances.
\end{inparaenum}
We have run the experiment with 80 clients and measured the request
latency.
We also ensured that no cache miss happens during our executions since we wanted
to solely measure the latency of \memcached{}, and not the data store attached to
it.

% \newcommand{\tabfont}{\small}
% \begin{table}[t]
% \footnotesize
% \centering
% \begin{tabular}{@{\hspace{0mm}\tabfont}c@{\hspace{1mm}\tabfont}c@{\hspace{1mm}\tabfont}c@{\hspace{1mm}\tabfont}c@{\hspace{-2mm}}}
% %   \hline\\[-5pt]
%
%   & \begin{tabular}{@{\hspace{0mm}\tabfont}c}Request\\
% 	latency
% 	\end{tabular}
%   & \begin{tabular}{@{\hspace{0mm}\tabfont}c}
%       Time to
%       add\\ instance
%     \end{tabular}
%   &
%     \begin{tabular}{@{\hspace{0mm}\tabfont}c}
%       Cost \\ (instance/h)
%     \end{tabular}\\[2pt]
%   \hline\\[-5pt]
%   \vspace{1em}
%   %  \hline
%   \aeon{} Memcached 	& 2.08ms & 1min & 0.032 \\
%   Amazon \ElastiCache{} &  1ms & % \begin{tabular}{@{\hspace{0mm}\tabfont}c}
%                             6min$\sim$% \\
%                               10min % \end{tabular}\vspace{1mm}
%   & 0.364\\
%   \hline
% \end{tabular}
% \caption{\aeon{} \Memcached{} vs. \ElastiCache{}}
% \label{table:memcached_comparison}
% \end{table}


We observed that on average, request latency in \aeon{} \memcached{} is two times
higher than Amazon ElastiCache: 2.08 ms in \aeon{} \memcached{} compared to
1ms in Amazon ElastiCache.
We note that cache.m3.xLarge instances are specifically tailored for Amazon
ElastiCache, and we believe that they play a crucial role in delivering such
low latency in Amazon ElastiCache. 
On the flipside, while adding a m1.xLarge instance to scale \aeon{} \memcached{}
takes around 1min, it takes around 6 to 10 mins to add a cache.m3.xLarge
instance for Amazon ElastiCache, which in applications with strong variations (in terms of frequency and extent) in workloads will likely lead to increased latencies when the system needs to scale out, and to increased costs when it needs to scale back in. 
The latter observation is particularly relevant as cache.m3.xLarge instances tailored for Amazon ElastiCache are
ten times more expensive than m1.xLarge instances (\$0.364/h vs. \$0.032/h ).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> ownership-check.tex <==
\subsection{Checking Ownership}
\label{sec:checking-ownership}

We consider a simple type-and-effect system to check that the
ownership network is indeed a DAG. 

\newcommand{\atcontext}{\Gamma}
\newcommand{\aceff}[1][]{C_{#1}}
% \newcommand{\aexp}{s}


The type-and-effect judgment for statements is of the form
\[\atcontext \vdash \aexp : \atype, \aceff\]
where, $\atcontext$ is a standard type environment, mapping variables
to their types, $\comm$ is a command, $\atype$ is the type of the
expression, and finally, $\aceff$ is a set of context class names,
which represent an over-approximation of the types of the context
instances manipulated by the expression. 

For method definitions the types are simply annotated with their
effects:
\[\atcontext \vdash  : \atype\ \amethod(\atype_0\ \avar_0, \dots,
\atype_n\ \avar_n) \{ \aexp \} : \bar{\atype}\]

And finally, for whole programs the type-and-effect system simply
checks that the ownership network is acyclic, and therefore the
type-and-effect system does not have a result. 

As in C (or Java), types of method definitions are assumed to be
given. Then we can simply obtain the type definition of a method by
consulting it's type as in $\mathsf{type}(\aclass, \amethod) =
\atype_0 \times \dots \times \atype_n\ \rightarrow\ \atype$

For the effect system, we will further add an effect to method
types. Hence, a method type has the form: 
$\mathsf{type}(\aclass, \amethod) =
\atype_0 \times \dots \times \atype_n\ \xrightarrow{\aceff}\ \atype$,
where as before, $\aceff$ is a set of context class names.

\begin{figure*}
  \centering
\[
\inferrule[]{
  \atcontext \vdash \aexp\ :\aclass,\ \aceff[0]\\
  \mathsf{type}(\aclass, f) = \atype_1 \times \dots \times \atype_n
  \xrightarrow{\aceff[n+1]} \atype\\\\
  \forall i\in[1,n],\ \atcontext \vdash e_i\ :\ \atype_i,\ \aceff[i]\\
  \aceff = \cup_{i \in [0,n+1]} \aceff[i]
}{
  \atcontext \vdash \aexp.f(\aexp_1, \dots, \aexp_n)\ :\ \atype,\ \aceff
}
\qquad
\inferrule[]{
  \atcontext \vdash \aexp\ :\acontext,\ \aceff[0]\\
  \mathsf{type}(\aclass, f) = \atype_1 \times \dots \times \atype_n
  \xrightarrow{\aceff[n+1]} \atype\\\\
  \forall i\in[1,n],\ \atcontext \vdash e_i\ :\ \atype_i,\ \aceff[i]\\
  \aceff = \cup_{i \in [0,n+1]} \aceff[i]
}{
  \atcontext \vdash \aexp.f(\aexp_1, \dots, \aexp_n)\ :\ \atype,\ \aceff
}
\]
\[
\inferrule[]{
  \atcontext \vdash \aexp_0\ :\ \atype_0,\ \aceff[0]\\
  \atcontext \vdash \aexp_1\ :\ \atype_1,\ \aceff[1]\\
}{
  \atcontext \vdash \aexp_0; \aexp_1\ :\ \atype_1,\ \aceff[0] \cup \aceff[1]\\
}{}
\qquad
\cdots
\qquad
\inferrule[]{
  \atcontext, \aval_0:\atype_0, \dots, \aval_0:\atype_0\
  \vdash\ \aexp\ :\ \atype,\ \aceff
}{
  \atcontext \vdash \atype\ \amethod(\atype_0\ \avar_0, \dots, \atype_n\ \avar_n) \{ \aexp \}\ : 
  \atype_0 \times \dots \times \atype_n \xrightarrow{\aceff} \atype
}
\]


  \[
  \inferrule[]
  {\mathcal{C} = \{\acontext \geq \acontext'\ |\ \acontext'\ \text{occurs in}\
    \Fields^*\ \text{or the effects in}\ \Methods^*\}}
  {\ctxtdec[\acontext]{}{\Fields^*}{\Methods^*}{\!\!} : \mathcal{C}}
  \qquad
  \inferrule[]
  {
    \mathcal{C}t = \{ \mathcal{C}\ |\ \acontext \in \Ctxts^*\ \&\
    \acontext : \mathcal{C}\}\\\
    \mathsf{topsort}(\mathcal{C}t) \neq \emptyset
  }
  {\Ctxts^*\ \Classes^*\ \mathtt{main}(\mathsf{args}) \{\
    \Statements^* \} : \checkmark}
  \]

  \caption{Checking DAG structure of ownership network}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> semantics.tex <==
% \section{Language}

% In this appendix we describe the major syntactic categories of \aeon{}
% and examples of their usage. 

% At top level we have programs $\Programs$ which are simply a list of
% context declarations $\Ctxts^*$, a list of classes declarations
% $\Classes^*$ and finally a single function $\mathsf{main}$ which
% represents the starting point of the program. 
% \paragraph{Contexts.} A context is declared using a unique name
% $\acontext$, and it comprises a list of contexts names ($\acontext^*$)
% representing the contexts it \emph{owns}.  
% % \gpnote*{Add the semantic interpretation of the lock of a context?}{ 
% While we do not enforce it
% at the syntactic level, it is an invariant of the ownership system
% that the ownership relation must constitute a directed acyclic graph
% (DAG) to avoid the possibility of deadlocks.
% % } 
% A context declaration provides each context with a name ($\acontext$)
% and contains a list of \emph{typed fields} $\Fields^*$ represented the
% data available in the context, and a number of \emph{methods}
% $\Methods^*$ that operate on these context fields.  
% % \gpnote[inline,nomargin]{Add here an explanation about: 1) synch/asynch methods, 2) locking to execute
% % methods, and 3) that context fields are not accessible other than
% % through the methods exported by the context, i.e., that fields are not
% % exported.
% % }  
% Contexts have global scope and are created statically.
% Contexts also provide a list of \emph{events}
% $\Event^*$, which can be called in the context. The implementation of
% events is similar to the implementation of normal methods, but their
% execution model is asynchronous, and each of them is guaranteed to
% execute atomically (i.e. in isolation w.r.t. other events). Unlike normal
% methods ($\Methods$) which represent a unity of functionality of a
% class or context, an event represents a request to the system (eg. a
% client accessing a website). The execution of events triggered by
% another event happens only after the termination of the calling
% one. More will be said about events later. The underlying assumption
% about contexts is that they encapsulate data that is closely
% related. We use contexts as the minimal unity of data (and
% functionality) that must reside in the same node of the network. As
% such, the migration of data necessary to achieve elasticity operates
% at the granularity of contexts.

\section{Semantics}
\label{sec:semantics}

In this section we present a formal semantics of a subset of the
\aeon{} language, which we shall call \aeoncore{}. The semantics of
\aeoncore{} will be described in two % \footnote{Three actually.}
stages. The former considers the executions that happen within a
context instance, without communication with other context instances, and the latter,
considers the synchronization of multiple context instances in the whole
system. 

\subsection{Intra-context semantics}
\label{sec:intra-cont-semant}

The first layer is a \emph{\bigstep{} semantics of a single context instance}
in isolation. Of course, this semantics can only make progress as long
as the currently executing event does not need to communicate with
other context instances. In essence, this semantics represents the atomic
evolution of a an event within the boundaries of actions requiring
communication. To formalize this semantics we introduce the following
syntactic categories: 
% \gp{I'm assuming that fields, methods and
%   variables are already defined.}  {
\[
\footnotesize
  \begin{array}{rcll}
    % \acontext, \acid & \in & \Contexts, \CID  & \text{{\sc Context(ID)}}\\
    % \avar & \in & \Vars & \text{{\sc Variables}}\\
    \aobj & \in & \Objects : \Fields \rightharpoonup \Vals& \text{{\sc Objects}}\\
    \aval & \in & \Vals \supseteq \Objects & \text{{\sc Values}}\\
    % \comm & \in & \Statements & \text{{\sc Commands}}\\
    \aheap & \in & \Heap : \Vars \rightharpoonup \Vals & \text{{\sc Store}}\\
    \alenv & \in & \LEnv : [\Vars \rightharpoonup \Vals] & \text{{\sc Local Env.}}\\
    \agenv & \in & \GEnv : \Vars \rightharpoonup \Vals & \text{{\sc Global Env.}}\\
    \aaccess & \in & \{\readonly, \exclusive \} & \text{{\sc Access Mode}}\\
    \acid & \in & \CID  & \text{{\sc Context ID}}\\
    % \achildren[] & \in & 2^{\CID} & \text{{\sc Children Set}}
\end{array}
\]
\noindent where we denote a list with square brackets.

Then, a configuration of this semantics is simply a tuple of the
form:\footnote{For readability we omit the method environment, which
  is also a static element of the intra-context configuration.}
\[\footnotesize (\aheap, \agenv, \alenv, \comm, \aaccess)\]

\begin{figure*}[t]
\renewcommand{\xrightarrow}[2]{\xhookrightarrow{#1}{#2}}
\centering
\footnotesize
\(
\inferrule[Sequence]
{
  (\aheap, \agenv,\alenv,\acmd_1, \aaccess)
  \xrightarrow{} 
  (\aheap', \agenv',\alenv',\cskip, \aaccess) 
}
{
  (\aheap, \agenv,\alenv,\acmd_1; \acmd_2, \aaccess)
  \xrightarrow{} 
  (\aheap', \agenv',\alenv',\acmd_2, \aaccess)
}
\hspace*{\fill}
  \inferrule[Synch Context Call]
  {\llbracket\vec{\avar}\rrbracket(\aheap,\agenv,\alenv) = \vec{\aval}\\
    \amethod\ \text{access mode is}\ \aaccess
  }
  {
    (\aheap,  \agenv, \alenv, \bvar
    :=\acontext[i].\amethod(\vec{\avar});\acmd_2, \aaccess)
    \xrightarrow{\lsynch[{\acontext[i]}]{\amethod}{\vec{\aval}}{\aaccess}}
    (\aheap,  \agenv, \alenv, \bvar :=\csuspend[{\acontext[i]}];\acmd_2, \aaccess)}
\)
\\[3pt]
\(
\inferrule[Sequence Label]
{
  (\aheap,\agenv,\alenv,\acmd_1, \aaccess) 
  \xrightarrow{\albl} 
  (\aheap',\agenv',\alenv',\acmd_1', \aaccess) 
}
{
  (\aheap,\agenv,\alenv,\acmd_1; \acmd_2, \aaccess) 
  \xrightarrow{\albl} 
  (\aheap',\agenv',\alenv',\acmd_1'; \acmd_2, \aaccess) 
}
\)
\hspace*{\fill}
\(
  \inferrule[ASynch Context Call]
  {\llbracket\vec{\avar}\rrbracket(\aheap,\agenv,\alenv) = \vec{\aval}\\
    \amethod\ \text{access mode is}\ \aaccess 
  }
  {
    (\aheap,  \agenv, \alenv, \mathsf{asynch}\ \acontext[i].\amethod(\vec{\avar});\acmd_2, \aaccess)
    \xrightarrow{\lasynch[{\acontext[i]}]{\amethod}{\vec{\aval}}{\aaccess}}
    (\aheap,  \agenv, \alenv, \mathsf{emit}; \acmd_2, \aaccess)}
\)
\hspace*{\fill}
\\[3pt]
{
\hspace*{\fill}
\(
  \inferrule[Field Update]
{
  \llbracket\avar\rrbracket(\aheap,\agenv,\alenv) = \aobj \\ 
  \llbracket e \rrbracket(\aheap,\agenv,\alenv) = \aval \\ 
  \aheap' = \aheap[\aobj.\afield \leftarrow \aval]
}
{
  (\aheap,\agenv,\alenv,\avar.\afield := e, {\color{red} \exclusive}) 
  \xrightarrow{} 
  (\aheap', \agenv,\alenv,\cskip, {\color{red} \exclusive}) 
}
\)
\hspace*{\fill}
\(
  \inferrule[Context Return]
  {|\alenv| = 1 }
  {
    (\aheap,  \agenv, \alenv, \mathsf{return}\ \aval;\acmd, \aaccess)
    \xrightarrow{\ret}
    (\aheap,  \agenv, \epsilon, \cskip, \aaccess)}
\)
\hspace*{\fill}
}
\caption{Intra-context \bigstep{} semantics}  
\label{fig:big-step}
\end{figure*}


Moreover, we add \emph{labels} which are used by the following
semantic level \emph{to synchronize} among multiple context instances. Labels
are sampled from the grammar:
\[
\footnotesize
  \begin{array}{lcl}
    \albl \in \Labels & ::= & \tau\ |\ \lret{\aval}\\
                      & | & \lsynch{\amethod}{\vec{\aval}}{\aaccess}\\
                      & | & \lasynch{\amethod}{\vec{\aval}}{\aaccess}\\
                      & | & \levent{\amethod}{\vec{\aval}}
  \end{array}
\]
\noindent where the $\tau$ label is silent, and shall generally be
omitted.  The label $\lsynch{\amethod}{\vec{\aval}}{\aaccess}$
indicates that the transition issues a synchronous call to context instance 
$\acid$ for method $\amethod$ and with arguments
$\vec{\aval}$. Moreover, the access mode is $\aaccess$. The meaning of
the other labels is self-explanatory.  Then, the judgment of this
semantics is of the form:
\[
\footnotesize
(\aheap, \agenv, \alenv, \comm, \aaccess) \xhookrightarrow{\albl}
(\aheap', \agenv', \alenv', \comm', \aaccess)
\]
\noindent The most important semantic rules of this level are shown in~\autoref{fig:big-step}.

As it can be seen from the {\sc Sequence} rule, this semantics encodes
a \bigstep{} evaluation provided that the corresponding command does
not emit a label other than $\tau$. The rule {\sc Sequence Label}
enforces that the execution is stopped at the point where the
semantics makes a labeled transition. The rule {\sc Field Update}
models filed assignments, and it requires that the access mode be
$\exclusive$, thus preventing readonly calls from modifying the
heap. We assume a given semantic function ($\llbracket\ \rrbracket$)
to evaluate expressions.  It is an error to write in a readonly call,
and the semantics simply defines no transitions for programs
attempting to do. Indeed, in \aeon{} a simple static analysis
checks that readonly methods never write. 

The rules for {\sc Synch} and {\sc ASynch Context Call} are similar
except for the event that they emit, and the \emph{place-holder command} that
they inject in the resulting configuration. 
In fact, we consider syntax for commands extended as follows  
\[
\footnotesize
\begin{array}{ccl}
  \comm \in \Statements & \ ::=\ & \dots\ |\ \csuspend[\acontext[]]\ |\ \cemit 
\end{array}
\]
\noindent where $\csuspend[\acontext[i]]$ and $\mathsf{emit}$ are
\emph{runtime commands} (they cannot appear in the source program),
used to indicate that a synchronization with another context instance is
necessary. Similarly, the fact that these commands emit an event represents that
this semantic layer will be stopped from making progress until the
label has been consumed by the rules of the inter-context semantics
which we will consider next. Since the semantics
of~\autoref{fig:big-step} does not provide rules for these runtime
commands, the execution will only be able to continue when they are
removed in the subsequent semantic layer.

Finally, {\sc Context Return} emits a return event on a return
statement only if the current local environment ($\alenv$) contains a
single call frame. This rule clears the local environment, where we
denote by $\epsilon$ the empty list.
The other rules are standard for sequential programming languages,
and are therefore ignored.

\subsection{Inter-context semantics}
\label{sec:inter-cont-semantics}

The second layer of our semantics considers the composition of all
context instances in the system.  We will use the following category to
indicate the type of requests made to a context instance:
\[
\footnotesize
\begin{array}{rcll}
  \adec \in \Dec & ::= & \mathsf{synch}\ |\ \mathsf{asynch}\ |\
                         \mathsf{event} & \text{{\sc Decorators}}
\end{array}
\]

Next, since there could be multiple readonly events executing their
methods in a single context instance, we need a pool of \emph{activations}
representing different threads executing readonly methods within a
context instance. Since each thread has their own local variable environment 
and code, we add this information into the activations. Moreover,
since at any point there could be at most one exclusive access
activation in a context instance, we use the activation set of a context instance
as lock. The definition of activations is as follows 
\[\footnotesize
\begin{array}{rcl}
  \aactivation \in \Activation & ::= & (\aeid, \aaccess, \adec, \alenv, \comm)\ |\ (\aeid, \aaccess, \bot)
\end{array}
\]
representing in the former case a running activation, and in the
latter, an activation that has terminated or is currently inactive in
this context instance, but whose lock cannot yet be safely removed.

The next ingredient we need to consider is the \emph{(request) queue} that each
context instance uses to buffer calls made to it. This queue will
contain requests sampled from the following syntax where we
assume that the metavariable $\aeid \in \EID$ represents an event ID:\\[2pt]
\centerline{
\(\begin{array}{rcl}
  % \aeid & \in & \EID \hspace*{\fill} \text{Event ID} \hspace*{\fill} \\[2pt]
  \areq\in \Requests & ::= & (\aeid, \amethod, \vec{\aval}, \adec, \aaccess)\ 
                             |\ \mathsf{lub\ }(\mathsf{event}\ \acid)
\end{array}\)
}\\[2pt]
% \[
% \footnotesize
% \begin{array}{rcl}
%   % \aeid & \in & \EID \hspace*{\fill} \text{Event ID} \hspace*{\fill} \\[2pt]
%   \areq\in \Requests & ::= & (\aeid, \amethod, \vec{\aval}, \adec, \aaccess)\ 
%                              |\ \mathsf{lub\ }(\mathsf{event}\ \acid)
% \end{array}
% \]
The former request represents a call from event $\aeid$ to method
$\amethod$ with decorator $\adec$, with arguments $\vec{\aval}$ and
access mode $\aaccess$. The latter denotes that an event executing in
context instance $\acid$ needs to lock the current context instance
(which is % happens to be 
the \lub{} of $\acid$). This latter request
serves only to lock the current context instance with the event, and the
response to this request is simply a notification to the event $\aeid$
in $\acid$ that the lock has been acquired, and execution can
begin. Then, a request queue is simply a list of requests, and it will
be ranged over with the metavariable
$\aqueue : [\Requests]$.\footnote{Recall that we denote a list with
  brackets.}

We are finally in a position to define context instances \emph{as considered
by this semantics}.
\[
\footnotesize \acontext \in \Ctxts ::= \{id:\CID,\ \aqueue :
[\Requests],\ \aheap:\Sigma,\ \agenv : \GEnv,\ A:2^{\Activation}\}\]
In this definition we use a record-like syntax, to name each of the
components of a context instance. Then, $\acontext.\aqueue$ represents the
queue of context instance $\acontext$.\footnote{By abuse of notation we will
  use the same convention for activations.} Moreover, we will use the
following notation for in-place update of the $\aheap$ component of
the $\acontext$:
\vspace{-5pt}
\[
\footnotesize
\acontext[][\aheap \leftarrow \aheap'].x =  
\begin{cases}
  \aheap' & \text{if}\ x = \aheap\\
  \acontext.x & \text{otherwise}
\end{cases}
\]
\noindent a similar convention applies to all other named components
of the context instance record. 

Finally, a configuration of the whole system is a pair
$(\aeventset, \acontextset)$ comprising a set of currently running
events $\aeventset \in 2^{\EID}$ and a set of context instances
$\acontextset \in 2^{\Ctxts}$ representing the ownership network.

The inter-context semantics, presented in~\autoref{fig:global-step}, is
given by judgments of the form 
\[
\footnotesize 
(\aeventset, \acontextset) \xrightarrow{} (\aeventset',
\acontextset')
\]

% \paragraph{The Composition Rules.}
\vspace{1mm}\noindent\textbf{Composition rules.}
Let us now consider the rules
of~\autoref{fig:global-step}. These rules are concerned with the
calling and returns of events and context calls. They ignore how an
event becomes \emph{activated} in a context instance, which will be discussed
in~\autoref{fig:activation}. 

% \gp{Currently using parent-child locking restriction.}
\begin{figure*}[!t]
  \centering
{
  \hspace*{\fill}
  \(
  \footnotesize
  \inferrule[Lift Intra]
  {
    (\acontext.\aheap, \acontext.\agenv, a.\alenv, a.\acmd, a.\aaccess) \xhookrightarrow{\ell}{}
    (\aheap', \agenv', \alenv', \acmd', a.\aaccess)\\
    \acontext.A = \mathcal{A} \cup \{a\}\\
    \acontext' = \acontext'[\aheap \leftarrow \aheap'][\agenv \leftarrow \agenv']
    \big[A \leftarrow \mathcal{A} \cup \{a[\alenv \leftarrow \alenv'][\acmd \leftarrow \acmd']\}\big]
  }
  {
    \acontext \xrightharpoondown{(\ell,a.\aeid)} \acontext'
  }
  \)
  \hspace*{\fill}
}
\\[5pt]
{
  \hspace*{\fill}
\(
  \footnotesize
  \inferrule[Synch Call]
  { 
    \acontext[1] \in \acontext[0].\acchild{}\\ 
    \acontext[0] \xrightharpoondown{(\lsynch[{\acontext[1]}]{\amethod}{\vec{\aval}}{\aaccess},\aeid)} \acontext[0]' \\\\
    \acontext[1]' = \acontext[1][\aqueue\leftarrow \aqueue \cdot
    (\aeid,\amethod,\vec{\aval},\syncm,\aaccess)]
  }
  {
    (\aeventset,\acontextset \cup \{\acontext[0],\acontext[1]\}) \xrightarrow{}
    (\aeventset,\acontextset \cup \{\acontext[0]',\acontext[1]'\})
  }
  \)
  \hspace*{\fill}
\(
\footnotesize
\inferrule[ASynch Call]
{ 
  \acontext[1] \in \acontext[0].\acchild{}\\ 
  \acontext[0]
  \xrightharpoondown{(\lasynch[{\acontext[1]}]{\amethod}{\vec{\aval}}{\aaccess},\aeid)}
  \acontext[0]' \\\\
  \acontext[0]'' = \acontext[0]'\big[\acmd \leftarrow \acontext[0]'.\acmd[{\color{blue}\mathsf{emit}}\leftarrow\cskip]\big]
  \\
  \acontext[1]' = \acontext[1][\aqueue\leftarrow \aqueue \cdot (\aeid,\amethod,\vec{\aval},\asyncm,\aaccess)]
}
{
  (\aeventset,\acontextset \cup \{\acontext[0],\acontext[1]\}) \xrightarrow{}
  (\aeventset,\acontextset \cup \{\acontext[0]'',\acontext[1]'\})
}
\)
  \hspace*{\fill}
}
\\[5pt]
{
\hspace*{\fill}
  \(
    \footnotesize
  \inferrule[Synch Return]
  { 
    \acontext[1] \xrightharpoondown{(\ret,\aeid)}{} \acontext[1]'\\
    \acontext[1].A = \mathcal{A}_1 \cup \{(\aeid, \aaccess, \_, \syncm, \_)\}\\
    % \acontext[0].A = \mathcal{A}_0 \cup \{(\aeid, \aaccess, \_, \syncm, \comm))\}\\
    \acontext[0].A = \mathcal{A}_0 \cup \{a\}\\
    a.\aeid = \aeid\\\\
    (\csuspend[\acontext[1]])\ \text{occurs in}\ a.\comm\\
    % a.\aaccess = \aaccess \quad a.\adec = \syncm\\
    \acontext[0]' = \acontext[0]\big[A \leftarrow \mathcal{A}_0 \cup
    \big\{a\big[\acmd \leftarrow
    a.\acmd[{\color{blue}(\csuspend[\acontext[1]])}\leftarrow
    v]\big]\big\}\big]\\
    \acontext[1]'' = \acontext'[A \leftarrow \mathcal{A}_1 \cup (\aeid,a.\aaccess, \bot)]
  }
  {
    (\aeventset,\acontextset \cup \{\acontext[0],\acontext[1]\}) \xrightarrow{}
    (\aeventset,\acontextset \cup \{\acontext[0]',\acontext[1]''\})
  }
  \)
\hspace*{\fill}
\(
\footnotesize
\inferrule[ASynch Return]
{ 
  \acontext[] \xrightharpoondown{(\ret,\aeid)}\acontext[]' \\
  \acontext[].A = \mathcal{A} \cup \{a\} \\   a.\aeid = \aeid\\
% \\ 
  a.\aaccess = \asyncm\\
  \acontext[]'' = \acontext'[A \leftarrow \mathcal{A} \cup (\aeid,a.\aaccess, \bot)]
}
{
  (\aeventset,\acontextset \cup \{\acontext[]\}) \xrightarrow{}
  (\aeventset,\acontextset \cup \{\acontext[]''\})\\\\
}
\)
\hspace*{\fill}
}
\\
{
\hspace*{\fill}
\(
\footnotesize
  \inferrule[Event Call UnShared]
  {\aeid \notin \aeventset \\
    \amethod\ \text{has access mode}\ \aaccess\ \text{in}\ \acontext\\\\
    \acontext = \mathsf{\lub{}}(\acontextset\cup\{\acontext\}, \acontext)\\ 
    \acontext' = \acontext[][\aqueue \leftarrow \acontext[].\aqueue \cdot
    (\aeid,\amethod,\vec{\aval},\mathsf{event},\aaccess)]
  }
  {(\aeventset,\acontextset \cup \{\acontext\}) \xrightarrow{}
    (\aeventset\cup\{\aeid\},\acontextset \cup \{\acontext'\})}
  \)
  \qquad \qquad
  \(
  \footnotesize
  \inferrule[Event Return \& Commit]
  { 
    \acontext[] \xrightharpoondown{(\ret,\aeid)}\acontext[]' \\
    \acontext[].A = \mathcal{A}\cup \{a\} \\\\
    a.\aeid = \aeid \\ a.\aaccess = \mathsf{event}\\
    \acontextset' = (\acontextset \cup \{\acontext[]'\})\downarrow\aeid
  }
  {
    (\aeventset,\acontextset \cup \{\acontext[]\}) \xrightarrow{}
    (\aeventset/\{\aeid\},\acontextset')
  }
\) 
\hspace*{\fill}
}
\\[5pt]
\(
\footnotesize
  \inferrule[Event Call Shared]
  { \aeid \notin \aeventset \\
    \amethod\ \text{has access mode}\ \aaccess\ \text{in}\ \acontext\\
    \acontext[\ell] = \mathsf{\lub{}}(\acontextset\cup\{\acontext\}, \acontext)\\\\
    \acontext[\ell] \neq \acontext \\
    \acontext[\ell]' = \acontext[\ell][\aqueue \leftarrow \acontext[\ell].\aqueue \cdot
    (\aeid,\amethod,\vec{\aval},\mathsf{lub}\ (\mathsf{event}\ \acontext),\aaccess)]
  }
  {(\aeventset,\acontextset \cup \{\acontext,\acontext[\ell]\}) \xrightarrow{}
    (\aeventset\cup\{\aeid,\},\acontextset \cup \{\acontext, \acontext[\ell]'\})}
\)
\caption{Global Rules (except activations)}
  \label{fig:global-step}
\end{figure*}

The rule {\sc Lift Intra} simply propagates the behavior of the
intra-context semantics of~\autoref{fig:big-step} by arranging the
elements of a context instance $\acontext$ and its activations as a
configuration of the semantics of~\autoref{fig:big-step}. Note that
this is the only rule to produce an arrow of the form
$\xrightharpoondown{(\albl, \aeid)}$ which is used in the premises of the other
rules. Moreover, notice that the label is simply propagated, with
the added information of the event emitting it. 

The rule {\sc Synch Call} considers the case where the intra-context
semantics emits a synchronous call label. This rule involves context instances
$\acontext[0]$ the source of the call, and $\acontext[1]$, its target
-- notice that we check that $\acontext[1]$ is a child of
$\acontext[0]$.\footnote{This check will be relaxed at the end of the
  section.}  As explained before, the only effect of this step is to
add the a request to the tail of $\acontext[1]$'s queue.

The rule {\sc Synch Return} in turn considers the case where a
synchronous call is terminated in $\acontext[1]$. In this case we
check that indeed an activation $a$ in $\acontext[0]$ is waiting for
the response of a synchronous call to $\acontext[0]$ (it is an
invariant that for each event, at most one activation is waiting for a
synchronous call from a single context instance). In that case, we substitute
the $\csuspend[\acontext[0]]$ command for the actual value produced by
the call, therefore allowing the semantics of~\autoref{fig:big-step}
to proceed. Notice that the activation is not removed from context instance
$\acontext[0]$ upon the return, but rather replaced with a $\bot$
marker. This is because this activation acts as a lock for the
context instance, and it will only be released upon the completion of the whole
event $\aeid$. % in the system.

The rule for {\sc ASynch Call} is similar to the one for {\sc
  Synch Call}, with the exception that the $\mathsf{emit}$
place-holder is immediately removed from the command of the issuing
context instance when the event is placed in the target's queue. This is
because the caller context instances needs not wait for the termination of the
callee, and so it's intra-context semantics can proceed. Consequently,
the rule for {\sc ASynch Return} is also simpler than its {\sc Synch}
counterpart, and in particular it involves a single context instance $\acontext[]$.

The next three rules consider the case of asynchronous event calls
issued to an event. The rule {\sc Event Call Unshared} considers the
case where the target context instance of the event, $\acontext[]$ is its own
dominator context instance (cf. the definition of~\autoref{sec:pmodel}). In
this case, no other context instances need to be contacted for locks, and
therefore all the rule does is to pick a \emph{fresh} event
identifier, $\aeid \notin \aeventset$, and add the event in the
context instance's queue. On the other hand, if the dominator  of $\acontext[]$
is another context instance $\acontext[\ell]$, the new event is added in the
queue of $\acontext[\ell]$ as a marker indicating that the context instance
$\acontext[\ell]$ has to be locked before the event starts
executing. Notice in rule {\sc Event Call Shared} that the target
context instance $\acontext$ is unmodified by the transition. 

The final rule in this figure is {\sc Event Return \& Commit}. This
rule simply removes the event ID $\aeid$ from the event set, and it
removes any activation appearing in any context instance for the event
$\aeid$. This is encoded with the notation
$\acontextset\downarrow\aeid$ defined as follows. 
\[
\footnotesize
\acontextset\downarrow\aeid = 
\begin{cases}
  \emptyset & \text{if}\ \acontextset = \emptyset\\
  \kern-5pt
\begin{array}{l}
  \acontextset'\downarrow\aeid\ \cup\\
  \kern5pt \{\acontext[0] [A\leftarrow(A/{\{(\aeid,\dots})\}]\} 
  \end{array}
  & % \kern-5pt
  \text{if}\
  \acontextset = \acontextset' \cup \{\acontext[0]\}
\end{cases}
\]
\noindent Notice that since we use activations as a lock, this
achieves the effect of removing the lock (either readonly or
exclusive) from all context instances that have been visited by the event
$\aeid$.\footnote{Evidently, the implementation of this rule requires
  communication between the dominator and all context instances affected by $\aeid$.}

% \paragraph{Activation Rules.}~ 
\vspace{1mm}\noindent\textbf{Activation rules.}
Let us now concentrate on the
activation rules show in~\autoref{fig:activation}, which dictate how
requests are removed from a context instance's queue, and scheduled for
execution.

\begin{figure*}[!ht]
\(
\footnotesize
  \hspace*{\fill}
  \inferrule[Exclusive Access]
  {
    \acontext.\aqueue = (\aeid, \amethod, \vec{\aval}, \adec, \exclusive) \cdot \aqueue' \\
    \acontext.A \subseteq \{(\aeid, \exclusive, \_, \_, \_)\}\\\\
    \acontext' = \acontext[][\aqueue \leftarrow \aqueue'][A \leftarrow
    \{(\aeid,\exclusive,\adec,\epsilon,\amthdenv(\amethod)(\vec{\aval}))\}] 
  }
  {
    (\aeventset, \acontextset \cup
    \{\acontext\}) 
    \xrightarrow{}
    (\aeventset, \acontextset \cup
    \{\acontext'\}) 
  }
  \)
  \hspace*{\fill}
\(
  \footnotesize
  \inferrule[LUB Lock and Schedule (Exclusive)]
  {
    \acontext[0].\aqueue = (\aeid, \amethod, \vec{\aval},
    \mathsf{lub}\ (\mathsf{event}\ \acontext[i]), \exclusive) \cdot
    \aqueue' \\
    \acontext[0].A = \emptyset\\\\
    \acontext[0]' = \acontext[0][\aqueue \leftarrow \aqueue']
    [A \leftarrow \{(\aeid,\exclusive,\bot)\}]\\
    \acontext[i]' = \acontext[i][\aqueue \leftarrow
    \acontext[i].\aqueue \cdot (\aeid, \amethod, \vec{\aval},
    \mathsf{event}, \exclusive)]
  }
  {
    (\aeventset, \acontextset \cup \{\acontext[0],\acontext[i]\}) 
    \xrightarrow{}
    (\aeventset, \acontextset \cup \{\acontext[0]',\acontext[i]'\}) 
  }
  \)
\\[5pt]
\(
  \footnotesize
  \inferrule[ReadOnly Access]
  {
    \acontext.\aqueue = (\aeid, \amethod, \vec{\aval}, \adec, \readonly) \cdot \aqueue' \\
    \exclusive \notin \acontext.A\\\\
    \acontext' = \acontext[][\aqueue \leftarrow \aqueue'][A \leftarrow
    \acontext.A \cup \{(\aeid,\readonly,\adec,\epsilon,\amthdenv(\amethod)(\vec{\aval}))\}]
  }
  {
    (\aeventset, \acontextset \cup
    \{\acontext\}) 
    \xrightarrow{}
    (\aeventset, \acontextset \cup
    \{\acontext'\}) 
  }
\hspace*{\fill}
 \inferrule[LUB Lock and Schedule (ReadOnly)]
  {
    \acontext[0].\aqueue = (\aeid, \amethod, \vec{\aval}, \mathsf{lub}\ (\mathsf{event}\ \acontext[i]), \readonly) \cdot
    \aqueue' \\
    \exclusive \notin \acontext[0].A\\\\
    \acontext[0]' = \acontext[0][\aqueue \leftarrow \aqueue']
    [A \leftarrow \{(\aeid,\readonly,\bot)\}]\\
    \acontext[i]' = \acontext[i][\aqueue \leftarrow
    \acontext[i].\aqueue \cdot (\aeid, \amethod, \vec{\aval},
    \mathsf{event}, \readonly)]
  }
  {
    (\aeventset, \acontextset \cup \{\acontext[0],\acontext[i]\}) 
    \xrightarrow{}
    (\aeventset, \acontextset \cup \{\acontext[0]',\acontext[i]'\}) 
  }
\)
\\[5pt]
% \gp{Explain this rule}\\
\(
\footnotesize
  \hspace*{\fill}
  \inferrule[Call Promotion]
  {\acontext.\aqueue = \aqueue_0 \cdot (\aeid, \aaccess, \dots) \cdot \aqueue_1\\
    \aeid\ \text{does not occur}\ \aqueue_0\\    
    (\aeid, \aaccess, \bot)\ \in \acontext.A\\
    \acontext[][\aqueue' \leftarrow (\aeid, \dots) \cdot \aqueue_0 \cdot \aqueue_1]
  }
  {(\aeventset, \acontextset \cup \{\acontext\}) 
  \xrightarrow{}
  (\aeventset, \acontextset \cup \{\acontext'\})
  }
  \hspace*{\fill}
\)

\caption{Activation rules}
\label{fig:activation}
\end{figure*}

The rules {\sc Exclusive Access} and {\sc ReadOnly Access} consult the
first request in the requests queue. In the former case, of the event
as $\exclusive$ access mode, the rule requires that the current
activation set of the context  instance($\acontext.A$) be empty,
meaning that there are not other events currently holding the
context instance. If the check is successful an activation is added for this
call, which will enable the {\sc Lift Intra} rule to start the
execution. Evidently, the head of the queue is removed. The latter
case simply checks that no $\exclusive$ activation is currently
present in the activation set. 

The {\sc LUB Lock and Schedule ...}  rules perform a similar check
in the \lub{} context instance, and upon successfully activating the event, they
simply forward the request to the target context instance (by adding it in its
queue). Notice that the activations added are of the form $(\aeid,
\aaccess, \bot)$ since the event does not execute in this context instance, but
the activation is only used as a lock. 

Finally, the {\sc Call Promotion} rule considers the case where a call
is made to a context instance that was already visited by the event
(i.e. $\aeid$ was already activated in the context instance). In this case, the
call can be executed regardless of other events that might have
arrived to the context instance,\footnote{Notice that this could only happen if
  the context instance $\acontext$ is its own dominator, since otherwise these
  events would not be queued in this context instance, but in its dominator
  instead.} and is therefore upgraded to the front of the requests
queue.

\begin{definition}
  We take the semantics of an \aeoncore{} program to be given as the
  transitive closure of the $\xrightarrow{}$ relation (denoted
  $\xrightarrow{}^*$) between configurations, starting with a given
  initial configuration $(\emptyset, \acontextset_{I})$ containing no
  events.
\end{definition}

\subsection{Meta-properties}
\label{sec:meta-properties}

In this section we develop the main claims about the high-level
semantics of \aeoncore{}.

% \paragraph{Deadlock Freedom.}~
\vspace{1mm}\noindent\textbf{Deadlock freedom.}
Let us begin by formally defining how deadlocks could manifest in
\aeoncore{}.

\begin{definition}[Deadlock State]
  \label{def:deadlock}
  We say a state $(\aeventset, \acontextset)$ contains a
  deadlock, if $\acontextset$ can be decomposed as:\\[2pt]
  \centerline{
    \( \acontextset = \acontextset' \cup \{\acontext[0], \acontext[1], \dots,
    \acontext[n]\} \)
  }\\[2pt]
  where for each $i \in [0,n]$ we have that there exists an event
  $\aeid[i] \in \aeventset$ such that: (i)
  $\aeid[i]\ \text{occurs in}\ \acontext[i].A$, and (ii)
  $\aeid[i]\ \text{occurs in}\ \acontext[i+1].\aqueue$, considering
  addition modulo $n$.
\end{definition}

A representation of a deadlock state is shown below, where the
context instances involved in the deadlock are marked with the primed names
($\acontext[0]'$, $\acontext[1]'$, $\acontext[2]'$). Notice that in
the queues of each of these context instances there is a request of an event
that is currently holding the previous context instance in the chain (shown
with incoming arrows marked $req(e_i)$), thus closing the
cycle.
\begin{center}
  \includegraphics[scale=.25]{figures/ddlock-crop}
\end{center}
\begin{theorem}
  The semantics of \aeoncore{} guarantees that no deadlock state can
  be reached.\footnote{Proofs are provided in~\autoref{sec:proofs}
  for reviewing.} 
\end{theorem}

% \begin{proof}({\sc Sketch}) The proof proceeds by contradiction
%   assuming that a first deadlock state $(\aeventset, \acontextset)$
%   can be reached. Firstly we observe that whenever an event is
%   executing in a context, it must be activated in its dominator. This
%   is an invariant preserved by the semantics of \aeoncore{}. Consider
%   now any of the contexts, say $\acontext[i]$, that is issuing a
%   request for event $\aeid[i]$ that is enqueued in the queue of a
%   context $\acontext[i+1]'$ in the deadlock cycle as shown in figure
%   above. Also, by the definition of deadlock we have that there is an
%   event $\aeid[i+1]$ that is currently holding the context
%   $\acontext[i+1]'$, and it's parent $\acontext[i+1]$. This, by the
%   definition of $\mathsf{share}$ of~\autoref{sec:ownership-network}
%   implies that they share a common dominator. Hence, by the
%   above mentioned invariant, they cannot be both executing, since at
%   most one of them is scheduled in the dominator context. This
%   contradiction proves the theorem.\footnote{The full proof is
%     provided in~\autoref{app:deadlock}.} 
% \end{proof}

% \paragraph{Linearizability.}~
\vspace{1mm}\noindent\textbf{Linearizability.}
Let us now show that the execution of \aeoncore{} events is
linearizable. We begin by stating some simple lemmas that are
necessary for the proof. 

% \begin{figure}[!t]
%   \vspace{-\topsep}
%   \centering
%     \begin{tikzpicture}[scale=0.3, every node/.style={scale=.9}]
%       \matrix (m) [matrix of math nodes,row sep=2em,column
%       sep=1.5em,minimum width=1.5em] {
%         & (\aeventset,\acontextset_0) \\
%         (\aeventset, \acontextset') &  & (\aeventset, \acontextset'') \\
%         & (\aeventset,\acontextset_1)\\};
%       \path[-stealth] 
%       (m-1-2) edge [dashed] node [left] {$\acontext[1]$} node [right] {$e_1$} (m-2-3) 
%       (m-2-3) edge [dashed] node [left] {$\acontext[0]$} node [right] {$e_0$} (m-3-2) 
%       (m-1-2) edge node [right] {$\acontext[0]$} node [left] {$e_0$} (m-2-1)
%       (m-2-1) edge node [right] {$\acontext[1]$} node [left] {$e_1$} (m-3-2);
%     \end{tikzpicture}  
%   \vspace{-2\topsep}
%   \caption{Commutativity of independent events}
%   \label{fig:commutativity}
% \end{figure}

% \begin{lemma}[Commutativity]
%   Consider two consecutive transitions where we assume two
%   contexts $\acontext[0], \acontext[1] \in \acontextset$, and two
%   events $e_0, e_1 \in \aeventset$:
%   \[\footnotesize
%   (\aeventset,\acontextset_0)
%     \underset{e_{0}}{\xrightarrow{\acontext[0]}} 
%     (\aeventset, \acontextset') 
%     \underset{e_{1}}{\xrightarrow{\acontext[1]}}
%     (\aeventset, \acontextset_1)\]
%   Here we denote with the arrow
%   $\underset{e}{\xrightarrow{\acontext[]}}$ the fact that the
%   transition involved the event identifier $e$ and it was performed in
%   the context $\acontext[]$.\footnote{Not to be confused with the
%     labels of Figures~\autoref{fig:big-step}-\autoref{fig:activation}.} We
%   have that either $\acontext[0] \neq \acontext[1]$ or $e_0.\aaccess =
%   e_1.\aaccess = \readonly$ and there exists an
%   intermediary context set $\acontextset''$ such that the following
%   transitions are also valid:
%   \[\footnotesize
%   (\aeventset, \acontextset_0) \underset{e_{1}}{\xrightarrow{\acontext[1]}}
%   (\aeventset, \acontextset'') \underset{e_{0}}{\xrightarrow{\acontext[0]}}
%   (\aeventset, \acontextset_1)\]
%   \autoref{fig:commutativity} depicts this lemma, where dashed arrows
%   represent the existential transitions required by the lemma. 
%   \label{lem:commutativity}
% \end{lemma}

% \begin{corollary}
%   \label{cor:push-forward}
%   Consider a sequence of transitions 
%   \[\footnotesize
%   \alpha\ =\ (\aeventset, \acontextset_0) \xrightarrow[e_0]{} 
%   (\aeventset, \acontextset_1) \xrightarrow[e_1]{}\ \dots\ \xrightarrow[e_{n-1}]{} 
%   (\aeventset, \acontextset_n)\]
%   where no step except the last one is a commit event. We can conclude
%   that there exists an equivalent trace 
%   \[\footnotesize
%   \alpha' = (\aeventset, \acontextset_0) \xrightarrow[\delta(e_{0})]{} 
%   (\aeventset, \acontextset'_1) \xrightarrow[\delta(e_{1})]{}\ \dots\ \xrightarrow[\delta(e_{n-1})]{} 
%   (\aeventset, \acontextset_n)\]
%   where $\delta$ is an bijection from $\{e_0, \dots, e_{n-1}\}$ to
%   itself, such that there exists an $m \in [0,n-1]$ with
%   (i) for all $i<m$ we have $\delta(e_i) = e_{m-1}$, and (ii) for each $i
%   \geq m$, $\delta(e_{i}) \neq e_{n-1}$. 
% \end{corollary}
% \noindent Essentially, the bijection $\delta$ pushes all transitions of
% $e_{n-1}$ to the front.  

\vspace{1mm}\noindent\textbf{Linear semantics of {\footnotesize\aeontitle{}}.}
% \paragraph{Linear semantics of \aeon{}.} 
We consider an alternative semantics of \aeon{}, given also by the
rules of~\autoref{fig:big-step},~\autoref{fig:global-step}
and~\autoref{fig:activation}, where we add the additional constraint
that there is at most one event activated in the context instance set
$\acontextset$. This essentially encodes a semantics of \aeon{}
where each event executes in complete isolation. Let us call this
the \emph{linear semantics of \aeon{}} and denote it with the special
arrow ``$\twoheadrightarrow$'' and denote context instance sets generated by
this semantics as $\hat{\acontextset}$.

The proof of linearizability shows that the \emph{linear semantics of
  \aeoncore{}} ($\twoheadrightarrow^*$) can simulate the semantics of
\aeoncore{} ($\xrightarrow{}^*$). To that end we consider a
simulation relation between configurations of the two different
semantics. We denote by $\mathcal{A}ct(\acontextset)$ the set of
events that are activated in any context instance of $\acontextset$.

\begin{definition}[Simulation Relation]
  We define the following simulation relation between a configuration
  of the linear semantics of \aeoncore{}, say
  $(\aeventset, \hat{\acontextset})$, with a configuration of the
  normal \aeoncore{}, say $(\aeventset, \acontextset)$, which we
  denote \((\aeventset, \hat{\acontextset})\ \mathcal{R}\ ( \aeventset,
  \acontextset)\) iff the following hold: % conditions are met:
  \begin{compactitem}
  \item[(i)] $\mathcal{A}ct(\hat{\acontextset}) = \emptyset$, and
  \item[(ii)] $(\aeventset, \hat{\acontextset}) \xrightarrow{*} (\aeventset, \acontextset')$
  \end{compactitem}
\end{definition}

Our simulation proof amounts to showing that the diagram below
commutes. 
\begin{center}
  \begin{tikzpicture}[scale=0.2, every node/.style={scale=.88}]
    \matrix (m) [matrix of math nodes,row sep=1.5em,column
    sep=4em,minimum width=2em] {
      (\aeventset, \hat{\acontextset}) & (\aeventset', \hat{\acontextset}') \\
      (\aeventset, \acontextset) & (\aeventset', \acontextset') \\};
    \path[-stealth] (m-1-1) edge [-] node [left] {$\mathcal{R}$}
    (m-2-1) edge [->>,dashed] node [above] {*} (m-1-2)
    (m-2-1.east|-m-2-2) edge (m-2-2) (m-1-2) edge [dashed,-] node
    [right] {$\mathcal{R}$} (m-2-2);
  \end{tikzpicture}  
\end{center}
\noindent That is to say, each time we start with a pair of similar
configurations, whenever the normal semantics of \aeoncore{} (the
low-level semantics) makes a step, the resulting configuration is
still related to the linear one, or there exist a number of steps in
the linear semantics that can simulate exactly the same
behavior.\footnote{Technically, a weak-simulation.} Notice in
particular, that the event sets $\aeventset$ in any two similar
configurations are identical, meaning that transitions that modify the
event set must be matched one-to-one.

\begin{theorem}[Simulation]
  \label{thm:sim}
  The relation $\mathcal{R}$ defined above is a weak-simulation from
  the normal (low-level) semantics of \aeoncore{} to the \emph{linear semantics} of
  \aeoncore{}.
\end{theorem}
\noindent The proof of this theorem is supported by a commutativity
argument between transitions corresponding to different
events (see~\autoref{lem:exclusive}).

% \begin{proof}({\sc Sketch}) The only interesting case of this proof is
%   the {\sc Return \& Commit} rule, which requires that the linear
%   semantics executes all the transitions of the event making the
%   commit in a single uninterrupted sequence. Then, the proof relies on
%   the fact that all contexts that have been visited by this event have
%   been locked since the beginning of the event, therefore no other
%   concurrent event could have modified their state (meaning that the
%   linear semantics configuration $\hat{\acontextset}$ coincides in
%   this context with the state in the normal semantics before the
%   execution of the committing event starting at $\acontextset$). Since
%   all context locks are taken in a tree-like fashion, and are not
%   released until commit, we have that the state of all these contexts
%   in the linear configuration coincides with the non-linear
%   configuration before the execution of the event. Moreover, they are
%   all free. Finally, by~\autoref{cor:push-forward} we know that we can
%   push the execution of this event forward, to conclude that the event
%   can be executed entirely from beginning to commit preserving the
%   exact same behavior. 
% \end{proof}

Evidently, \emph{the simulation induces a linearizability proof},
where events are linearized at their commit point. 

\begin{corollary}[Linearizability]
  Since the linear \emph{semantics of \aeoncore{}} is linear, and
  it does not reorder non-overlapping events, \autoref{thm:sim}
  implies that the semantics of \aeoncore{} enforces linearizability
  of events. 
\end{corollary}

\subsection{Relaxing the direct-owner restriction}

Notice that calls could be issued from a context instance to any descendent 
context instance, provided that locks are acquired in a
top-down hand-in-hand fashion (this is required to guarantee
deadlock freedom). But then, allowing the runtime system to perform
the locking automatically on a path from the caller to the destination
context instance allows us to remove the parent-to-child restriction, and in
particular, since locks are acquired only once for each event,
subsequent calls can directly traverse the context instance network without
accessing all intermediate descendants. To model that behavior we use an asynchronous ``runtime'' locking rule, which simply takes
the lock of a context instance when the runtime best believes that it will be
necessary following the above mentioned top-down hand-in-hand policy. 
\[
\inferrule[Auto Lock] 
{
  \acontext[1] \in \acontext[0].\acchild{}\\
  (\aeid, \aaccess, \dots) \in \acontext[0].A\\\\
  \aaccess = \readonly \Rightarrow \exclusive\ \text{not in}\ \acontext[1].A\\
  \aaccess = \exclusive \Rightarrow \acontext[1].A = \emptyset\\\\
 \acontext[1]' = \acontext[1][a \leftarrow (\aeid, \aaccess, \bot)]\\
}
{
  (\aeventset, \acontextset \cup \{\acontext[0], \acontext[1]\})
  \xrightarrow{}
  (\aeventset, \acontextset \cup \{\acontext[0], \acontext[1]'\})
}
\]
This rule allows us to relax the constraint
$\acontext[1] \in \acontext[0].\acchild{}$ in the {\sc Call} rules for
$\acontext[1] \in \mathsf{desc}(\acontextset\cup\{\acontext[0],
\acontext[1]\}, \acontext[0])$, and 
hence, allows any context instance to call any of its descendant context instances.\footnote{In fact, it even allows bottom-up calls provided
  that the required context instances are already locked, and therefore not
  subject to further deadlocks.}

% \gp{This is all optional.}

\begin{comment}

\subsection{Checking ownership}
\label{sec:checking-ownership}

We consider a simple type-and-effect system to check that the
ownership network is indeed a DAG. 

\newcommand{\atcontext}{\Gamma}
\newcommand{\aceff}[1][]{C_{#1}}
% \newcommand{\aexp}{s}

The type-and-effect judgment for statements is of the form
\[\atcontext \vdash \aexp : \atype, \aceff\]
where, $\atcontext$ is a standard type environment, mapping variables
to their types, $\comm$ is a command, $\atype$ is the type of the
expression, and finally, $\aceff$ is a set of context class names,
which represent an over-approximation of the types of the context
instances manipulated by the expression. 

For method definitions the types are simply annotated with their
effects:
\[\atcontext \vdash  : \atype\ \amethod(\atype_0\ \avar_0, \dots,
\atype_n\ \avar_n) \{ \aexp \} : \bar{\atype}\]

And finally, for whole programs the type-and-effect system simply
checks that the ownership network is acyclic, and therefore the
type-and-effect system does not have a result. 

As in C (or Java), types of method definitions are assumed to be
given. Then we can simply obtain the type definition of a method by
consulting it's type as in $\mathsf{type}(\aclass, \amethod) =
\atype_0 \times \dots \times \atype_n\ \rightarrow\ \atype$

For the effect system, we will further add an effect to method
types. Hence, a method type has the form: 
$\mathsf{type}(\aclass, \amethod) =
\atype_0 \times \dots \times \atype_n\ \xrightarrow{\aceff}\ \atype$,
where as before, $\aceff$ is a set of context class names.

\begin{figure*}
  \centering
\[
\inferrule[]{
  \atcontext \vdash \aexp\ :\aclass,\ \aceff[0]\\
  \mathsf{type}(\aclass, f) = \atype_1 \times \dots \times \atype_n
  \xrightarrow{\aceff[n+1]} \atype\\\\
  \forall i\in[1,n],\ \atcontext \vdash e_i\ :\ \atype_i,\ \aceff[i]\\
  \aceff = \cup_{i \in [0,n+1]} \aceff[i]
}{
  \atcontext \vdash \aexp.f(\aexp_1, \dots, \aexp_n)\ :\ \atype,\ \aceff
}
\qquad
\inferrule[]{
  \atcontext \vdash \aexp\ :\acontext,\ \aceff[0]\\
  \mathsf{type}(\aclass, f) = \atype_1 \times \dots \times \atype_n
  \xrightarrow{\aceff[n+1]} \atype\\\\
  \forall i\in[1,n],\ \atcontext \vdash e_i\ :\ \atype_i,\ \aceff[i]\\
  \aceff = \cup_{i \in [0,n+1]} \aceff[i]
}{
  \atcontext \vdash \aexp.f(\aexp_1, \dots, \aexp_n)\ :\ \atype,\ \aceff
}
\]
\[
\inferrule[]{
  \atcontext \vdash \aexp_0\ :\ \atype_0,\ \aceff[0]\\
  \atcontext \vdash \aexp_1\ :\ \atype_1,\ \aceff[1]\\
}{
  \atcontext \vdash \aexp_0; \aexp_1\ :\ \atype_1,\ \aceff[0] \cup \aceff[1]\\
}{}
\qquad
\cdots
\qquad
\inferrule[]{
  \atcontext, \aval_0:\atype_0, \dots, \aval_0:\atype_0\
  \vdash\ \aexp\ :\ \atype,\ \aceff
}{
  \atcontext \vdash \atype\ \amethod(\atype_0\ \avar_0, \dots, \atype_n\ \avar_n) \{ \aexp \}\ : 
  \atype_0 \times \dots \times \atype_n \xrightarrow{\aceff} \atype
}
\]


  \[
  \inferrule[]
  {\mathcal{C} = \{\acontext \geq \acontext'\ |\ \acontext'\ \text{occurs in}\
    \Fields^*\ \text{or the effects in}\ \Methods^*\}}
  {\ctxtdec[\acontext]{}{\Fields^*}{\Methods^*}{\!\!} : \mathcal{C}}
  \qquad
  \inferrule[]
  {
    \mathcal{C}t = \{ \mathcal{C}\ |\ \acontext \in \Ctxts^*\ \&\
    \acontext : \mathcal{C}\}\\\
    \mathsf{topsort}(\mathcal{C}t) \neq \emptyset
  }
  {\Ctxts^*\ \Classes^*\ \mathtt{main}(\mathsf{args}) \{\
    \Statements^* \} : \checkmark}
  \]

  \caption{Checking DAG structure of ownership network}
\end{figure*}
\end{comment}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> sriv.tex <==
 \begin{algorithm}[h]
\begin{algorithmic}[1]
  \State {\bf assert} (this.context = {\bf LUB}($e$.target))
  \For{(c $\in \mathsf{Reachable}$($e$.target))}
  \State lock\_queue[c].enqueue($e$.eid)
  \EndFor
  \State $e$.target.enqueue(e)
\end{algorithmic}  
\caption{Lock\_LUB and schedule event $e$}
\end{algorithm}

{\bf GP: We assume that each context has a map from contexts to a queue
  of event IDs representing the events that attempt to lock that context.}
\begin{algorithm}[h]
\begin{algorithmic}[1]
  \For{(c $\in \mathsf{Reachable}$($e$.target))}
  \State lock\_queue[c].dequeue()
  \EndFor
\end{algorithmic}  
\caption{UNLOCK\_LUB and schedule event $e$}
\end{algorithm}

{\bf GP: LUB responds to lock request.}
\begin{algorithm}[h]
\begin{algorithmic}[1]
  \State wait(lock\_queue[C].top == $e$.eid)
  \State {\bf Respond} ``success'' {\bf to C}
\end{algorithmic}  
\caption{LUB response to lock by event $e$ on context C}
\end{algorithm}

{\bf GP: How to execute an event in a context C}
\begin{algorithm}[h]
\begin{algorithmic}[1]
  \State req = C.queue.dequeue()
  \State lock = req.ev.lub.sendLockRequest(C)
  \State wait(lock == ``success'')
  \State req.execute()
\end{algorithmic}  
\caption{Dequeue and execute in context C}
\end{algorithm}

\begin{algorithm}[h]
\caption{Event $e$ to $\mathsf{lock[r]}$ context $C$ from $C'$}
\begin{algorithmic}[1]
	 	\If{$(C\neq C') \wedge (C'\in \textit{Contexts}(\mathsf{Dom})) 
		  \wedge (\mathsf{Dom}(C)\neq \mathsf{Dom}(C'))$}
		  %\Comment{Get owner permission}
		  \State \textbf{Send} $\ms{msg}(\ms{LOCK[r]},C,e)$ to $\mathsf{Dom}(C')$
		  \State \hspace{10mm}\textbf{Wait for response from} $\mathsf{Dom}(C')$
		  %\Comment{Get children}
		  \State \textbf{Send} $\ms{msg}(\ms{LOCK[r]},C,e)$ to $\mathsf{Dom}(C)$
		  \State \hspace{10mm}\textbf{Wait for response from} $\mathsf{Dom}(C)$
		  
		 \Else
		  \State $\ms{msg}(\ms{LOCK}[r],C,e)$ to $\mathsf{Dom}(C)$
		  \State \hspace{10mm}\textbf{Wait for response from} $\mathsf{Dom}(C)$
		\EndIf
\end{algorithmic}
\end{algorithm}% \begin{figure}[h]

\begin{algorithm}[H]
\caption{\textbf{Receive} $\ms{msg}(\ms{LOCK},C,e)$ \textbf{from} process $p_j$; code for process $p_i$ }
\begin{algorithmic}[1]
	 	\If{$\lit{req}(\ms{LOCK},e)\in \ms{Queue}(C)$}
		  \If{$\lit{req}(\ms{LOCK},e)=\ms{Queue}(C).\lit{front}()$}
		        \State \textbf{Send lock response to} $p_j$
		   \ElsIf{$\lit{req}(\ms{LOCK},e).\ms{Mode}='r'$}
			\ForAll{$\lit{req}\in \ms{Queue}(C)$}
			  \If{$\lit{req}.\ms{Mode}='r' \wedge \lit{req}.\ms{Event}='e'$}
			      \State \textbf{Send lock response to} $p_j$
			     
			   \ElsIf{$\lit{req}.\ms{Mode}='w'$}
			      \State \textbf{Block}
			   \EndIf
			\EndFor
			    
		   \EndIf
		   
		 \ElsIf{$\lit{req}(\ms{VLOCK},e)\in \ms{Queue}(C)$}
		    \State \textbf{Replace with} $\lit{req}(\ms{LOCK},e)$
		  \ElsIf{$\lit{req}(\ms{UNLOCK},e)\in \ms{Queue}(C)$}
		    \State \textbf{Replace with} $\lit{req}(\ms{LOCK},e)$
		  \Else
		    \State $\ms{Queue}(C).\lit{add}(\lit{req}(\ms{LOCK},e))$
		    
		\EndIf
		\ForAll{$C'\in \ms{Contexts}(p_i)$}
		  \If{$C =\lit{owner}(C')$}
		    \State $\ms{Queue}(C').\lit{add}(\lit{req}(\ms{VLOCK},e))$
		   \EndIf
		 \EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\caption{\textbf{Receive} $\ms{msg}(\ms{UNLOCK},C,e)$ \textbf{from} process $p_j$; code for process $p_i$ }
\begin{algorithmic}[1]
	 	\State \textbf{Replace} $\lit{req}(\ms{LOCK},e)$ \textbf{with} $\lit{req}(\ms{UNLOCK},e)$ \textbf{in}
	 	$\ms{Queue}(C)$
	 	\ForAll{$\{C_n,C_m \} \in \ms{Contexts}(p_i)$}
		  \If{$C_n=\lit{owner}(C_m)$}
		    \State $\ms{Contexts}(p_i).\lit{Swap}(C_n,C_m)$
		  \EndIf
		\EndFor
		\ForAll{$C'\in \ms{Contexts}(p_i)$}
		  
		  \If{$\lit{req}(\ms{UNLOCK},e)\in \ms{Queue}(C')$}
		    \If{$\mathsf{Dom}(C')\neq p_i$}
		      \State \textbf{Send} $\ms{msg}(\ms{UNLOCK},C',e)$ to $\mathsf{Dom}(C')$
		     \EndIf
		  \State $\ms{Queue}(C').\lit{remove}(\lit{req}(\ms{UNLOCK},e))$
		  
		  \ElsIf{$\lit{req}(\ms{VLOCK},e)\in \ms{Queue}(C')$}
		    \State $\ms{Queue}(C').\lit{remove}(\lit{req}(\ms{VLOCK},e))$
		   
		  \ElsIf{$\lit{req}(\ms{LOCK},e)\in \ms{Queue}(C')$}
		    \State \textit{goto} Line~\ref{line:rel}
		  \EndIf
		\EndFor
		\ForAll{$C'\in \ms{Contexts}(p_i)$} \label{line:rel}
		    \ForAll{$\lit{req} \in \ms{Queue}(C')$}
		  	  \If{$\lit{req}=\ms{Queue}(C).\lit{front}() \wedge \lit{req}.\ms{Mode}='w'$}
			      \State \textbf{Send lock response to} $\lit{seq}.\ms{proc}$
			      \State \textbf{break and continue}
			   \ElsIf{$\lit{req}.\ms{Mode}='r'$}
			      \State \textbf{Send lock response to} $\lit{seq}.\ms{proc}$
			    \ElsIf{$\lit{req}.\ms{Mode}='w'$}
			      \State \textbf{break and continue}
			    \EndIf
		    \EndFor
		 \EndFor
			
		    
		  
\end{algorithmic}
\end{algorithm}% \begin{figure}[h]

